Black-box Off-policy Estimation for Infinite-Horizon Reinforcement Learning

Off-policy estimation for long-horizon problems is important in many real-life applications such as healthcare and robotics, where high-fidelity simulators may not be available and on-policy evaluation is expensive or impossible. Recently, \cite{liu18breaking} proposed an approach that avoids the \emph{curse of horizon} suffered by typical importance-sampling-based methods. While showing promising results, this approach is limited in practice as it requires data be drawn from the \emph{stationary distribution} of a \emph{known} behavior policy. In this work, we propose a novel approach that eliminates such limitations. In particular, we formulate the problem as solving for the fixed point of a certain operator. Using tools from Reproducing Kernel Hilbert Spaces (RKHSs), we develop a new estimator that computes importance ratios of stationary distributions, without knowledge of how the off-policy data are collected. We analyze its asymptotic consistency and finite-sample generalization. Experiments on benchmarks verify the effectiveness of our approach.

==> final/body.tex <==

\section{Introduction}\label{sec:intro}

As reinforcement learning (RL)  %\cite{sutton18reinforcement} 
is increasingly applied to crucial real-life problems like robotics, recommendation and conversation systems, off-policy estimation becomes even more critical. The task here is to estimate the average long-term reward of a target policy, given historical data collected by (possibly unknown) behavior policies. Since the reward and next state depend on what action the policy chooses, simply averaging rewards in off-policy data does not estimate the target policy's long-term reward.  Instead, proper correction must be made to remove the bias in data distribution.

%such off-policy data collected by behavior policies cannot be directly used to estimate the target policy's long-term reward.

One approach is to build a simulator that mimics the reward and next-state transitions in the real world, and then evaluate the target policy against the simulator~\cite{fonteneau13batch,ie19recsim}. While the idea is natural, building a high-fidelity simulator could be extensively challenging in numerous domains, such as those that involve human interactions. Another approach is to use propensity scores as importance weights, so that we could use the weighted average of rewards in off-policy data as a suitable estimate of the average reward of the target policy. The latter approach is more robust, as it does not require modeling assumptions about the real world's dynamics.  It often finds more success in short-horizon problems like contextual bandits, but its variance often grows exponentially in the horizon, a phenomenon known as ``the curse of horizon''~\cite{liu18breaking}.
%
%Off-policy evaluation is important in many applications where simulators are not available.  Building a simulated model is risky in not being able to control modeling bias.  Most of previous works rely on (nearly) unbiased inverse propensity score methods, which have found successes in short-horizon problems like recommendation.  But in long-horizon problems, their effectiveness is limited by the curse of horizon.

To address this challenge, \cite{liu18breaking} proposed to solve an optimization problem of a minimax nature, whose solution directly estimates the desired propensity score of states \emph{under the stationary distribution}, avoiding an explicit dependence on horizon. While their method is shown to give more accurate predictions than previous algorithms, it is limited in several important ways:
%
\begin{itemize}
%
\item{The method requires that data be collected by a known behavior policy. In practice, however, such data are often collected over an extended period of time by multiple, unknown behavior policies.  
%Furthermore, in many situations, the behavior policy may be unknown.  
For example, observational healthcare data typically contain patient records, whose treatments were provided by different doctors in multiple hospitals, each following potentially different procedures that are not always possible to specify explicitly.}
%
\item{The method requires that the off-policy data reach the stationary distribution of the behavior policy.  In reality, it may take a very long time for a trajectory to reach the stationary distribution, which may be impractical due to various reasons like costs and missing data.}

%\qiang{it seems our current method also requires infinite horizon? since it solves a fixed point?} 
%\lihong{Yes, but this point is that our prev method requires dataset must have reached stationary.}
%
\end{itemize}
%As will shown later, both assumptions are critical to the success of the method of \cite{liu18breaking}.

In this paper, we introduce a novel approach for the off-policy estimation problem that overcome these drawbacks. The main contributions of our work are three-fold:
\begin{itemize}
    \item We formulate the off-policy estimation problem into one of solving for the fixed point of an operator. Different from the related, and similar, Bellman operator that goes forward in time, this operator is backward in time.
    \item We develop a new algorithm, which does not have the aforementioned limitations of \cite{liu18breaking}, and analyze its generalization bounds.  Specifically, the algorithm does not require that the off-policy data come from the stationary distribution, or that the behavior policy be known.
    %In particular and unlike \cite{liu18breaking}, our method does not require to estimate the behavior policy.
    \item We empirically demonstrate the effectiveness of our method on several classic control benchmarks. In particular, we show that, unlike \cite{liu18breaking}, our method is effective even if the off-policy data has not reached the stationary distribution.
\end{itemize}
In the next section, we give a brief overview of recent and related works. We then move to describing the problem setting that we have used in the course of the paper and our off-policy estimation approach. Finally, we present several experimental results to show the effectiveness of our method.

\paragraph{Notation.}
In the following, we use $\Simplex(\Xset)$ to denote the set of distributions over a set $\Xset$. The $\ell_2$ norm of vector $x$ is $\norm{x}$. Given a real-valued function $f$ defined on some set $\Xset$, let $\norm{f}_2 \defeq \sqrt{\int_\Xset f(x)^2 dx}$.
Finally, we denote by $[n]$ the set $\{1,2,\ldots,n\}$, and $\one{A}$ the indicator function.  

\section{Related works}\label{sec:related}

Our work focuses on estimating a scalar (average long-term reward) that summarizes the quality of a policy and has extensive applications in practice. This is different from value function or policy learning from off-policy data~\cite{precup01off,maei10toward,sutton16emphatic,munos16safe,metelli18policy}, where the major goal is to ensure stability and convergence. Yet, these two problems share numerous core techniques, such as importance reweighting and doubly robustness. Off-policy estimation and evaluation can also be used as a component for policy optimization~\cite{jiang16doubly,gelada19off,liu19off,zhang19generalized}.

%Regression estimator: estimate $P$ and $R$ from $\Dset$, then solve $M=\langle \Sset, \Aset, \hat{P}, \hat{R}\rangle$ for $\rho_\pi$.  Low variance, but uncontrolled bias.  Example: \cite{fonteneau13batch}

Importance reweighting, or inverse propensity scoring, has been used for off-policy RL~\cite{precup01off,murphy01marginal,li15minimax,munos16safe,hanna17bootstrapping,xie19optimal}. Its accuracy can be improved by various techniques~\cite{jiang16doubly,thomas16data,guo17using,farajtabar18more}. However, these methods typically have a variance that grows exponentially with the horizon, limiting their application to mostly short-horizon problems like contextual bandits~\cite{dudik11doubly,bottou13counterfactual}.  
%Doubly robust: combines regression estimator and IPS estimator, may reduce variance, but still suffer the curse of horizon~.  Also discuss \cite{xie19optimal}.

There have been recent efforts to avoid the exponential blow-up of variance in basic inverse propensity scoring.  A few authors explored the alternative to estimate the propensity score of a state's \emph{stationary distribution}~\cite{liu18breaking,gelada19off}, when behavior policies are known. Later, \cite{nachum2019dualdice} extended this idea to situations with \emph{unknown} behavior policies. However, their approach only works for the discounted reward criterion. In contrast, our work considers the more general and challenging \emph{undiscounted} criterion. In the next section, we briefly mention the setting under which we study this problem and then present our {\em black-box} off-policy estimator.
%\lihong{Check Peter's behavior policy search and Emma papers.}

%The approach of \cite{nachum2019dualdice} requires $\gamma<1$.  Also \cite{gelada19off}.   The approach of \cite{nachum2019dualdice} (maybe \cite{gelada19off}) requires $\gamma<1$.  Approximating with $\gamma \approx 1$ does not work well (to be verified by experiments).

Our black-box estimator is inspired by previous work for black-box importance sampling~\cite{liu17black}.  Interestingly, the authors show that it is beneficial to estimate propensity scores from data without using knowledge of the behavior distribution (called proposal distribution in that paper), \emph{even if} it is available; see also \cite{henmi07importance} for related arguments.
%This result is similar in style to Theorem~3.2 of \cite{feng2019kernel}, but is based on using a different operator.
Similar benefits may exist for our black-box off-policy estimator developed here, although a systematic study is outside  the scope of this paper. 

\section{Problem Setting}\label{sec:setting}

Consider a Markov decision process (MDP)~\cite{puterman94markov} $M=\langle \Sset, \Aset, P, R, p_0, \gamma \rangle$, where $\Sset$ and $\Aset$ are the state and action spaces, $P$ is the transition probability function, $R$ is the reward function, $p_0\in\Simplex(\Sset)$ is the initial state distribution, and $\gamma\in[0,1]$ is the discount factor. A policy $\pi$ maps states to a distribution over actions: $\pi:\Sset\mapsto\Simplex(\Aset)$, and $\pi(a|s)$ is the probability of choosing action $a$ in state $s$ by policy $\pi$. With a fixed $\pi$, a trajectory $\tau=(s_0,a_0,r_0,s_1,a_1,r_1,\ldots)$ is generated as follows:\footnote{For simplicity in exposition, we assume rewards are deterministic. However, everything in this work generalizes directly to the case of stochastic rewards.}
\[
s_0 \sim p_0(\cdot), \quad a_t \sim \pi(\cdot|s_t), \quad r_t = R(s_t,a_t), \quad s_{t+1} \sim P(\cdot|s_t,a_t), \quad \forall t \ge 0\,.
\]

Given a \emph{target} policy $\pi$, we consider two reward criteria, undiscounted $(\gamma=1)$ and discounted ($\gamma<1$), where $\E_{\pi}[\cdot]$ indicates the trajectory $\tau$ is controlled by policy $\pi$:
\begin{eqnarray}
%
\text{(undiscounted)} \qquad & \rho_\pi & \defeq \lim_{T\to\infty}\E_{\pi}\left[\frac{1}{T}\sum_{t=1}^T r_t\right] = \E_{(s,a)\sim d_\pi}[r]\,, \label{eqn:polval} \\
%
\text{(discounted)} \qquad & \rho_{\pi,\lambda} & \defeq
(1-\gamma) \E_{\pi}\left[\sum_{t=0}^\infty \gamma^t r_t \right]\,. \label{eqn:polval_disc}
%\E_{\pi}\left[\frac{1}{T}\sum_{t=1}^T r_t\right] = \E_{(s,a)\sim d_\pi}[r]\,. \label{eqn:polval_disc}
%
\end{eqnarray}
In the above, $d_\pi$ is the stationary distribution over $\SAset$, which exists and is unique under certain assumptions~\cite{levin17markov}.

The $\gamma<1$ case can be reduced to the undiscounted case of $\gamma=1$, but not vice versa. Indeed, one can show that the discounted reward in \eqref{eqn:polval_disc} can be interpreted as the stationary distribution of an induced Markov process, whose transition function is a mixture of $P$ and the initial-state distribution $p_0$. We refer interested readers to \appref{sec:reward-reduction} for more details. Accordingly, in the following and without the loss of generality, we will merely focus on the more general undiscounted criterion in \eqref{eqn:polval}, and suppress the unnecessary dependency on $p_0$ and $\gamma$.

%\qiang{any missing references for black-box related papers, other than \cite{liu17black}?}

In the off-policy estimation problem, we are interested in estimating $\rho_\pi$ for a given target policy $\pi$. However, instead of having access to on-policy trajectories generated by $\pi$, we have a set of $n$ transitions collected by some unknown (i.e., ``{\em black-box}'' or behavior-agnostic~\cite{nachum2019dualdice}) behavior mechanism $\pibeh$:
\[
\Dset \defeq \{(s_i, a_i, r_i, s_i')\}_{1 \le i \le n}\,.
\]
Therefore, the goal of off-policy estimation is to estimate $\rho_\pi$ based on $\Dset$, for a given target policy $\pi$. 

The setting we described above is quite general, covering a number of situations. For example, $\pibeh$ might be a single policy and $\Dset$ might consist of one or multiple trajectories collected by $\pibeh$. In this special case, $s_i'=s_{i+1}$ for $1<i<n$; this is the off-policy RL scenario widely studied~\cite{precup01off, sutton16emphatic, munos16safe, liu18breaking, gelada19off}. Furthermore, if $\pibeh=\pi$, we recover the on-policy setting. On the other hand, $\pibeh$ and $\Dset$ can consist of multiple policies and their corresponding trajectories. In this situation, unlike the single policy case $s_i'$ and $s_{i+1}$ might originate from two distinct policies. In general, one can consider $\pibeh$ as a distribution over $\SAset$ where $(s_i,a_i)$ in $\Dset$ are sampled from. Having introduced the general setting of the problem, we will describe our estimation approach in the next section.
% m or simply a distribution over $\SAset$ where $(s_i,a_i)$ in $\Dset$ are sampled from.
%\lihong{Is it (mathematically) too vague?}


\section{Black-box estimation}\label{sec:bb}
%\todo{QL: I worry some people may feel the backward flow operator is self is not (mathematically) new. since people use it often,  sometimes implicitly. for example, our infinite horizon also used it? should we emphasize black box instead?}
%Since the target policy $\pi$ is given and fixed, we suppress the notation $\pi$ in the following to simplify notation.

Our estimator is based on the following operator defined on functions over $\SAset$. For discrete state-action spaces, given any $d\in\Rset^{\SAset}$,
\begin{equation}
\Bpi d(s,a) \defeq \pi(a|s) \sum_{\xi\in\Sset,\alpha\in\Aset} P(s|\xi,\alpha) d(\xi,\alpha)\,. \label{eqn:bbop}
\end{equation}
While we will develop the rest of the paper using the discrete version above for simplicity, the continuous version can be similarly obtained without affecting the estimator and results: 
% \ali{Lihong, please take a look at the word "result"}
\begin{equation}
\Bpi d(s,a) = \pi(a|s) \int_{\xi,\alpha} \mathrm{d}P(s|\xi,\alpha)d(\xi,\alpha)\,, \label{eqn:bbop-c}
\end{equation}
where $P$ is now interpreted as the transition kernel.

We should note that $\Bpi$ is indeed different from the Bellman operator~\cite{puterman94markov}; although they have some similarities. In particular, given some state-action pair $(s,a)$, the Bellman operator is defined using next state $s'$ of $(s,a)$, while $\Bpi$ is defined using \emph{previous} state-actions $(\xi,\alpha)$ that \emph{transition to} $s$. It is in this sense that $\Bpi$ is backward (in time). Furthermore, as we will show later, $d$ has the interpretation of a distribution over $\SAset$. Therefore, $\Bpi$ describes how visitation \emph{flows} from $(\xi,\alpha)$ to $(s,a)$ and hence, we call it the \emph{backward flow} operator. Note that similar forms of $\Bpi$ have appeared in the literature, usually used to encode constraints in a dual linear program for an MDP~\cite{wang08stable,wang17primal,dai18boosting}. However, the application of $\Bpi$ for the off-policy estimation problem as considered here appears new to the best of our knowledge.

An important property of $\Bpi$ is that, under certain assumptions, the stationary distribution $d_\pi$ is the unique fixed point that lies in $\Simplex(\SAset)$~\cite{levin17markov}:
\begin{equation}\label{eqn:bop-fp}
d_\pi = \Bpi d_\pi \quad \text{and} \quad d_\pi \in \Simplex(\SAset)\,. 
\end{equation}
This property is the key element we use to derive our estimator as we describe in the following.

\subsection{Black-box estimator}

In most cases, off-policy estimation involves a weighted average of observed rewards $r_i$ in $\Dset$. We therefore aim to directly estimate these (non-negative) weights which we denote by $w=\{w_i\}\in\Simplex([n])$; that is, $w_i \ge 0$ for $i\in[n]$ and $\sum_{i=1}^n w_i = 1$. Note that the normalization of $w$ may be ensured by techniques such as self-normalized importance sampling~\cite{liu01monte}. 
%for $i\in[n]$.  Suppose $w\in\Simplex([n])$ (say, as in self-normalized importance sampling), that is, $w_i \ge 0$ and $\sum_{i=1}^n w_i = 1$.  
Once such a $w$ is obtained, the estimated reward is given by:
\begin{equation}
%\hat{\rho}_\pi = \frac{\sum_{i=1}^n w_i r_i}{\sum_{i=1}^n w_i}\,. \label{eqn:bb-ips}
\hat{\rho}_\pi = \sum_{i=1}^n w_i r_i \,. \label{eqn:bb-ips}
\end{equation}
%
%Suppose $w=\{w_i\}\in\Simplex([n])$, that is, $w_i \ge 0$ and $\sum_{i=1}^n w_i = 1$.  Then, 
Effectively, any $w\in\Simplex([n])$ defines an empirical distribution which we denote by $d_w$ over $\SAset$:
\begin{equation}
d_w(s,a) \defeq \sum_{i=1}^n w_i \one{s_i=s,a_i=a}\,.  \label{eqn:bb-dw}
\end{equation}
Equation~\ref{eqn:bb-ips} is equivalent to $\hat{\rho}_\pi = \E_{(s,a)\sim d_w}[r]$.
Comparing it to \eqref{eqn:polval}, we naturally want to optimize $w$ so that $d_w$ is close to $d_\pi$. Therefore, inspired by the fixed-point property of $d_\pi$ in \eqref{eqn:bop-fp}, the problem naturally becomes one of minimizing the discrepancy between $d_w$ and $\Bpi d_w$.  In practice, $w$ is often represented in a parametric way:
\begin{align}\label{eqn:bb-param}
w_i = \tilde{w}_i / \sum_l \tilde{w}_l\,, \qquad
\tilde{w}_i \defeq W(s_i,a_i;\omega) \ge 0\,,
\end{align}
where $W(.)$ is a parametric model, such as neural networks, with parameters $\omega\in\Omega$. We have now reached the following optimization problem:
\begin{equation}
\min_{\omega\in\Omega} \Dist{d_w}{\Bpi d_w}\,, \label{eqn:bb-opt}
\end{equation}
where $\Dist{\cdot}{\cdot}$ is some discrepancy function between distributions.
In practice, $\Bop$ is unknown, and must be approximated by samples in the dataset $\Dset$:
\[
\Bpihat d_w(s,a) \defeq \pi(a|s) \sum_{i=1}^n w_i ~ \1\{s_i'=s\} \,.
\]
%and similarly for \eqref{eqn:bbop-c}.  
Clearly, $\Bpihat d_w$ is a valid distribution over $\SAset$ induced by $w$ and $\Dset$, and the black-box estimator solves for $w$ by minimizing $\Dist{d_w}{\Bpihat d_w}$.

\subsection{Black-box estimator with MMD}

There are different choices for $\Dist{\cdot}{\cdot}$ in \eqref{eqn:bb-opt}, and multiple approaches to solve it~\cite{nguyen10estimating,dai17learning}.
%with $\Bpi$ approximated by empirical data  
%In other words, instead of the stationary distribution $d_\pi$, we use samples from the training data to approximate $\Bpi$}. 
%
Here, we describe one such algorithm based on Maximum Mean Discrepancy (MMD)~\cite{muandet17kernel}. For simplicity, the discussion in this subsection assumes $\SAset$ is finite, but the extension to continuous $\SAset$ is immediate.

Let $\kk(\cdot,\cdot)$ be a positive definite kernel function defined on $(\SAset)^2$.
Given two real-valued functions, $f$ and $g$, defined on $\SAset$ we define the following bilinear functional
\begin{equation}
\kkf{f}{g} \qquad \defeq \sum_{(s,a)\in\SAset, (\sbar,\abar)\in\SAset} f(s,a) \,\cdot\,\kk\left((s,a),(\sbar,\abar)\right) \,\cdot\,g(\sbar,\abar)\,. \label{eqn:kkf}
\end{equation}
Clearly, we have $\kkf{f}{f} \geq 0$ for any $f$ due to the positive definiteness of $\kk$.  
In addition, $\kk$ is called \emph{strictly integrally positive definite} if $\kkf{f}{f} = 0$ implies $\norm{f}_2 = 0$.  

Let $\mathcal H$ be the reproducing kernel Hilbert space (RKHS) associated with the kernel function $\kk$. 
This is the unique Hilbert space that includes functions that can be expressed as a sum of countably many terms: $f(\cdot)=\sum_i u^i ~ \kk((s^i,a^i), \cdot)$, where $\{u^i\}\subset \mathbb R$, and $\{(s^i,a^i)\}\subseteq \SAset$. The space $\Hset$ is equipped with an inner product defined as follow: given $f,g\in\Hset$ such that $f=\sum_i u^i~\kk((s^i,a^i), \cdot)$ and $g=\sum_i v^i~\kk((s^i,a^i), \cdot)$, the inner product is $\langle f, g\rangle_{\Hset} \defeq \sum_{i,j} u^i v^j ~\kk(s^i,a^i), (s^j, a^j))$, 
%for $g(\cdot)=\sum_i v_i ~\kk((s^i,a^i), \cdot)$, and 
which induces the norm defined by $\norm{f}_{\mathcal H} \defeq \sqrt{\sum_{i,j} u^i u^j \kk((s^i,a^i), (s^j, a^j))}$.
%In addition, 
%where 
%\rev{
%and $\Hset$ the associated reproducing kernel Hilbert space (RKHS). \textbf{[[[[An intuition or some light background about %RKHS?]]]]} Given a real-valued function $f$ defined on $\SAset$ such that
%\[
%\norm{f}_2 \defeq \sum_{(s,a)\in\SAset} f(s,a)^2 < \infty\,,
%\]
%its corresponding \emph{RKHS norm} in $\Hset$ is given by
%\textbf{[[[[Use $\norm{f}_\Hset$ instead?]]]]}
%\lihong{No need to assume $f \not \equiv 0$?}
%\lihong{Continuous case?} 
%\qiang{Should we start "denote $(s,a)$ by $x$ and $(\sbar,\abar)$ by $\xbar$ for simplicity" here?}
%\lihong{Maybe too early, as $K_{ij}$ requires to take $s$ and $a$ separately?}
%the kernel $\kk(x,x')$ is strictly integrally positive definite, in that 
%$$\kkf{f}{f} \defeq \sum_{(s,a)\in\SAset, (\sbar,\abar)\in\SAset} f(s,a)\kf((s,a),(\sbar,\abar)) f(\sbar,\abar)\,.$$
%Clearly, $\kkf{f}{f}>0$ as long as $f \not \equiv 0$.}
%for any $f\not\equiv 0$ and $\norm{f}_2:=\sum_{s,a}{f(s,a)^2} <\infty$.  
%Moreover, denote by $\Hset$ the corresponding reproducing kernel Hilbert space (RKHS).
%Then, we have 

Given $\Hset$, the maximum mean discrepancy between two distributions, $\mu_1$ and $\mu_2$, is defined by
\begin{equation*}
    \DistMMD{\mu_1}{\mu_2} 
\defeq \sup_{f\in\Hset}
\left\{\E_{\mu_1}[f] - \E_{\mu_2}[f], 
~~~~~\text{s.t.} \quad \norm{f}_\Hset\le1
\right\}\,.
\end{equation*}
Here, $f$ may be considered as a discriminator, playing a similar role as the discriminator network in generative adversarial networks~\cite{goodfellow14generative}, to measure the difference between $\mu_1$ and $\mu_2$. 
%\begin{eqnarray*}
%    \DistMMD{d_w}{\Bpihat d_w} 
%&=& \sup_{f\in\Hset}
%\left\{\E_{d_w}[f] - \E_{\Bpihat d_w}[f], 
%~~~~~\text{s.t.} \quad \norm{f}_\Hset\le1
%\right\}\,,
%%&=& \kkf{d_w}{d_w} - 2\kkf{d_w}{\Bpihat d_w} + \kkf{\Bpihat d_w} {\Bpihat d_w}\,.
%\end{eqnarray*}
A useful property of MMD is that it admits a closed-form expression~\cite{gretton2012kernel}:
\begin{align*} 
\DistMMD{\mu_1}{\mu_2} 
& = \kkf{\mu_1-\mu_2}{\mu_1-\mu_2} \\
& = \kkf{\mu_1}{\mu_1}
- 2 \kkf{\mu_1}{\mu_2}  
+ \kkf{\mu_2}{\mu_2}\,, 
\end{align*}
%\begin{eqnarray*}
%    \DistMMD{\mu_1}{\mu_2} 
%&=& \kkf{d_w}{d_w} - 2\kkf{d_w}{\Bpihat d_w} + %\kkf{\Bpihat d_w} {\Bpihat d_w}\,. 
%\end{eqnarray*}
where $\kkf{\cdot}{\cdot}$ is defined in \eqref{eqn:kkf},
and we used the bilinear property $\kkf{\cdot}{\cdot}$. 
Interested readers are referred to surveys~\cite{berlinet2011reproducing, muandet2017kernel} for more background on RKHS and MMD.

Applying MMD to our objective, % and realizing that $\kkf{\cdot}{\cdot}$ is bilinear in its arguments, 
we have
\begin{eqnarray*}
    \DistMMD{d_w}{\Bpihat d_w} 
%&=& \kkf{d_w-\Bpihat d_w}{d_w-\Bpihat d_w} \\
%&=& \sup_{f\in\Hset}
%\left\{\E_{d_w}[f] - \E_{\Bpihat d_w}[f]
%~~~~~s.t.~~~~~\norm{f}_\Hset\le1
%\right\} \\
&=& \kkf{d_w}{d_w} - 2\kkf{d_w}{\Bpihat d_w} + \kkf{\Bpihat d_w} {\Bpihat d_w}\,. 
\end{eqnarray*}

%where we define 
%\[
%\kkf{d}{\bar{d}~} \defeq \E_{(s,a)\sim d}\E_{(\bar{s},\bar{a})\sim\bar{d}}\left[\kf((s,a),(\bar{s},\bar{a}))\right]\,.
%\]
In the above, both $d_w$ and $\Bpihat d_w$ are simply probability mass functions on a finite subset of $\SAset$, consisting of state-actions encountered in $\Dset$.
%With straightforward calculations, 
It follows immediately from \eqref{eqn:kkf} that
\begin{eqnarray*}
\kkf{d_w}{d_w} &=& \sum_{i,j} w_i w_j \underbrace{\kf((s_i,a_i),(s_j,a_j))}_{K^{(0)}_{i,j}} \\
\kkf{d_w}{\Bpihat d_w} &=& \sum_{i,j} w_i w_j \underbrace{\sum_{a'} \pi(a'|s_j') \kf((s_i,a_i),(s_j',a'))}_{K^{(1)}_{i,j}} \\
\kkf{\Bpihat d_w} {\Bpihat d_w} &=& \sum_{i,j} w_i w_j \underbrace{\sum_{a_i',a_j'}\pi(a_i'|s_i')\pi(a_j'|s_j') \kf((s_i',a_i'),(s_j',a_j'))}_{K^{(2)}_{i,j}}.
\end{eqnarray*}
Defining $K_{i,j} \defeq K^{(0)}_{i,j} -2 K^{(1)}_{i,j} + K^{(2)}_{i,j}$, we can express the objective as a function of $\omega$ (since $\{w_i\}$ depends on $\omega$; see \eqref{eqn:bb-param}):
\begin{equation}\label{eq:loss_kernel}
\ell(\omega) = \sum_{i,j} w_i w_j K_{i,j} \,.
%W(s_i,a_i;\omega) W(s_j,a_j;\omega) K_{i,j}\,.
\end{equation}

\begin{remark}
Mini-batch training is an effective approach to solve large-scale problems. However, the objective $\ell(\omega)$ is not in a form that is ready for mini-batch training, as $w_i$ requires normalization (\eqref{eqn:bb-param}) that involves \emph{all} data in $\Dset$. Instead, we may equivalently minimize $L(\omega) \defeq \log\ell(\omega)$, which can be turned into a form that allow mini-batch training, using a trick that is also useful in other machine learning contexts~\cite{jean15using}. See
\appref{sec:bb-minibatch} for more details.
\end{remark}

Algorithm~\ref{alg:bb} in Appendix \ref{sec:ps-code} summarizes our estimator.  We next present theoretical analysis of our approach. We show the consistency of our result and provide a sample complexity bound.



\subsection{Theoretical Analysis}

%\textcolor{red}{LL: regarding notation, how about keeping $\Dist{}{}$ for general discrepancy function as in \eqref{eqn:bb-opt}, while using $\D_\kk$ for the MMD objective (defined in Sec 4.2)?}

\paragraph{Consistency.} The following theorem shows that the exact minimizer of \eqref{eqn:bb-opt} coincides with the fixed point of $\Bpi$, and the objective function measures the norm of the estimation error %($d-d_\pi$) 
in an induced RKHS. 
To simplify exposition, we
assume $x = (s,a)$ and $x' = (s',a')$ 
a successive action-state pair following $x$: $x' \sim  d_\pi(\cdot~|~x)$, where 
$d_\pi(x'~|~x)$ is the transition probability from $x$ to $x'$, that is, $d_\pi(x'~|~x) = 
P(s'~|~s,a) \pi(a'|s')$. 
%use the shorthand $(x,x')$ with $x=(s,a)$ and $x'=(s', a')$ to represent a successive action-state transition pair, similarly for 
Similarly, we denote by $(\bar x, \bar x')=((\bar{s},\bar{a}),~ (\bar{s}',\bar{a}'))$ %to represent 
 an independent copy of $(x, x').$
%$\bar{x}=(\bar{s},\bar{a})$ and $\bar{x}'= (\bar{s}',\bar{a}')$. 
%and similarly for $x' = (\bar{s}, \bar{a})$ and $\bar{x}'$.

%For simplicity, 
%\begin{ass} \label{ass:uniqueness}
%Assume that
%\end{ass}

%We provide the p%r
%We provide a theoretical justification of our metric $D(d_w ~||~ \Bpi d_w)$ by showing that it controls 
\begin{thm}
Suppose $\kk$ is strictly integrally positive definite, and $d_\pi$ is the unique fixed point of $\Bpi$ in \eqref{eqn:bop-fp}. %$\Simplex(\SAset)$.%Assumption~\ref{ass:uniqueness} hold.
%1) the kernel $\kk(x,x')$ is strictly integrally positive definite, in that 
%$$
%\kkf{\delta}{\delta} = \sum_{x} \delta(x)\kk(x,\bar x) \delta(\bar x) >0
%$$ 
%for $\delta\not\equiv 0$ and  $\norm{\delta}_2:=\sum_x{\delta(x)^2} <\infty$, and 
%
%2) the true visitation distribution $d_\pi$ is the unique solution of the fixed point equation $d = \Bpi d$.  
%
Then, for any $d\in\Simplex(\SAset)$,
%\lihong{This thm applies to all $d\in\Simplex(\SAset)$, not just $d_w$ in \eqref{eqn:bb-dw}?} 
%\lihong{$\Dist{d_w}{\Bpi d_w}$?}
\[
\D_\kk (d~||~\Bpi d) = 0 \quad\Longleftrightarrow\quad d = d_\pi\,.
\]
Furthermore, $\D_\kk(d~||~\Bpi d)$ equals an MMD between $d$ and $d_\pi$, with a transformed kernel: %in fact
%\lihong{$\Dist{}{}$ or $\D_\kk$?}
$$
\D_\kk(d~||~\Bpi d) = \D_{\tilde \kk} (d ~||~ d_\pi)\,,
$$
where $\tilde \kk(x, {\bar x)}$ is a positive definite kernel, defined by 
$$
\tilde \kk(x,{\bar x}) = 
\E_{\pi}[\kk(x,\bar x) -\kk(x,\bar x') - \kk(x',\bar x) + \kk(x',\bar x') ~|~(x, \bar x)],
%\kk(x,\bar x) - \mathcal P_\pi^{x} \kk(x,\bar x) - \mathcal P_\pi^{\bar x} \kk(x,\bar x) + \mathcal P_\pi^{x} \mathcal P_\pi^{\bar x}  \kk(x,\bar x), 
$$
where the expectation is 
with respect to $x' \sim d_\pi(\cdot ~|~ x)$ and $\bar x'\sim d_{\pi}(\cdot ~|~ \bar x)$, with 
 $x'$ and $\bar x'$ drawn independently. 
 %Here $d_\pi$ 
\label{thm:consistency}
\end{thm}  
%$$\mathcal P_\pi^x \kk(x,\bar x) = \sum_{x'} P_\pi(x'|x) \kk(x,\bar x).  $$
%
%\qiang{This result is similar in style to Theorem~3.2 of \cite{feng2019kernel}, but is based on using a different operator.}

\paragraph{Generalization.} 
We next give a sample complexity analysis. In practice, 
the estimated weight $\hat w$ is based on minimizing the empirical loss
$\D_\kk(d_w~||~\hat \Bpi d_w)$, where $\Bpi$ is replaced by the empirical approximation $\hat \Bpi$. 
The following theorem compares the empirical weights 
$\hat w$ with the \emph{oracle weight} $w_*$ obtained by minimizing the expected loss $\D_\kk(d_w~||~\Bpi d_w)$, with the exact transition operator $\Bpi$. 

%It is desirable to understand how $\hat w$ compares with the oracle estimator $w_* := \arg\min_{w\in \mathcal W}\D_\kk(d_w~||~\Bpi d_w)$, the minimizer of the loss with the exact transition operator $\Bpi$. 

%In order to have a proper generalization bound, we need to sufficiently constraint the set $\mathcal W$  of possible weight functions. To do so, we 

%there is a function $w(x,x')$, such that $w_i = w(x_i,x_i')/n$, where $n$ introduced so that $w(x_i,x_i') = O(1)$. 
%(as a special case, we find it is convenient to assume $w_i = w(x_i)/n$, so that $w$ does not dependent on $x'$).  

\begin{thm}
\label{thm:generalization}
Assume the weight function is decided by $w_i =  W(s_i, a_i; ~ \omega)/n$. Denote by $\mathcal W = \{\tilde W(\cdot; ~ \omega) \colon\omega \in \Omega \}$ the model class of $W(\cdot; \omega)$. 
%\lihong{$\tilde{W}$ or $W$?} 
Assume $
\hat w $ is the minimizer of the empirical loss 
$\D_\kk(d_w~||~\hat \Bpi d_w)$
and $w^*$ the minimizer of expected loss $\D_\kk(d_w~||~\Bpi d_w)$. % are %the empirical and oracle estimators, respectively. 
Assume $\{x_i\}_{i=1}^n$ are i.i.d. samples. 
Then, with probability $1-\delta$ we have
\begin{align*} 
\D_\kk(d_{\hat w} ~||~ \Bpi d_{
\hat w}) 
- \D_\kk(d_{w_*} ~||~ \Bpi d_{ w_*}) \leq  
 16 r_{\max} \mathcal R_n(\mathcal W) +  
 \frac{16 r_{\max}^2   + r_{\max}^2\sqrt{8\log(1/\delta)}}{\sqrt{n}}, 
\end{align*} 
where $\mathcal R_n(\mathcal W)$ denotes the expected Rademacher complexity of $\mathcal W$ with data size $n$, and 
$r_{\max} \defeq \max(\norm{\mathcal W}_\infty, \sup_{x} \sqrt{\kk(x,x)})$,    with $\norm{\mathcal W}_\infty:= \sup\{\norm{W}_\infty \colon W\in \mathcal W\}.$
%As 
%Theorem~\ref{thm:generalization}
This suggests a generalization error of $O(1/\sqrt{n})$ if $\mathcal R_n(\mathcal W) = O(1/\sqrt{n})$, 
which is typical for parametric families of functions.  
\end{thm}

%\textcolor{red}{
%The assumption of $w_i =  W(s_i, a_i; ~ \omega)/n$ is made so that the weights $w_i$ are $O(1/n)$ while the function $ W(s_i, a_i; ~ \omega)$ are $O(1)$. }


% \newpage
\section{Experiments}\label{sec:exp}

In this section, we present experiments to compare the performance of our proposed method with other baselines on the off-policy evaluation problem. In general and for each experiment, we use a behavior policy $\pi_{\rm BEH}$ to generate trajectories of length $T_{\rm BEH}$. We then use these generated samples from a behavior policy to estimate the expected reward of a given target policy $\pi$. To compare our approach with other baselines, we use the root mean squared error (RMSE) with respect to the average long-term reward of the target policy $\pi$.  The latter is estimated using a trajectory of length $T_{\rm TAR} \gg 1$.  In particular, we compare our proposed {\em black-box} approach with the following baselines:

\begin{itemize}
    \item {\em naive averaging} baseline in which we simply estimate the expected reward of a target policy by averaging the rewards over the trajectories generated by the behavior policy.
    \item {\em model-based} baseline where we use the kernel regression technique with a standard Gaussian RBF kernel. We set the bandwidth of the kernel to the median (or \nth{25} or \nth{75} percentiles) of the pairwise euclidean distances between the observed data points.
    \item{ \em inverse propensity score (IPS)} baseline introduced by \cite{liu18breaking}. 
\end{itemize}

We will first use a simple MDP from \cite{thomas16data} to highlight the IPS drawback we previously mentioned in Section \ref{sec:intro}.
%; that is in IPS off-policy data should reach the stationary distribution while our proposed approach does not need that. 
We then move to classical control benchmarks. %For each problem, we briefly describe the task and then present results on how each method performs on the off-policy evaluation problem as we described above.

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figs/modelwin.eps}
         \caption{ModelWin MDP from \cite{thomas16data}.}
         \label{fig:modelwin_a}
     \end{subfigure}
    \hspace{0.15\textwidth}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figs/modelwin_new.png}
         \caption{The RMSE of different methods as we change the length of horizon w.r.t the target policy reward. IPS depends on the horizon length while our method is independent of the horizon length.}
         \label{fig:modelwin_b}
     \end{subfigure}
    
\end{figure}


\iffalse
\begin{figure}
\centering
\subfigure(a){\includegraphics[width=0.25\textwidth]{Figs/modelwin.eps}}
\subfigure(b){\includegraphics[width=0.3\textwidth]{Figs/modelwin_new.png}}
\caption{(a) ModelWin MDP from \cite{thomas16data}. (b) The RMSE of different methods as we change the length of horizon w.r.t the target policy reward. IPS depends on the horizon length while our method is independent of the horizon length.}
\label{fig:modelwin}
\end{figure}
\fi

\subsection{Toy Example}
The {\em ModelWin} domain first introduced in \cite{thomas16data} is a fully observable MDP with three states and two actions as denoted in Figure \ref{fig:modelwin_a}. The agent always begins in $s_1$ and should choose between two actions $a_1$ and $a_2$. If the agent chooses $a_1$, then with probability of $p$ and $1-p$ it makes a transition to $s_2$ and $s_3$ and receives a reward of $r=1$ and $r=-1$, respectively. On the other hand, if the agent chooses $a_2$, then with probability of $p$ and $1-p$ it makes a transition to $s_3$ with the reward of $r=-1$ and $s_2$ with the reward of $r=1$, respectively. Once the agent is in either $s_2$ or $s_3$, it goes back to the $s_1$ in the next step without any reward. In our experiments, we set $p=0.4$.

We define the behavior and target policies as the following. In the target policy, once the agent is in $s_1$, it chooses $a_1$ and $a_2$ with the probability of 0.9 and 0.1, respectively. On the other hand and for the behavior policy, once the agent is in $s_1$, it chooses $a_1$ and $a_2$ with the probability of 0.7 and 0.3, respectively. We calculate the average on-policy reward from samples based on running a trajectory of length $T_{\rm TAR}=50,000$ collected by the target policy. We estimate this on-policy reward using trajectories of length $T_{\rm BEH}\in\{4,8,16,32,64,128\}$ collected by the behavior policy. In each case, we set the number of trajectories such that the total number of transitions (i.e., $T_{\rm BEH}$ times the number of trajectories) is kept constant. For example, for $T_{\rm BEH}=4$ and $T_{\rm BEH}=8$ we use 50,000 and 25,000 trajectories, respectively. Since the problem has finitely many state-actions, we use the tabular method and hence, \eqref{eq:loss_kernel} turns into a quadratic programming. We then report the result of each setting based on 10 Monte-Carlo samples.

As we can see in Figure \ref{fig:modelwin_b}, the naive averaging method performs poorly consistently and independent of the length of trajectories collected by the behavior policies. On the other hand, IPS performs poorly when the collected trajectories have short-horizon and gets better as the horizon length of trajectories get larger. 
This is expected for IPS --- as mentioned in Section \ref{sec:intro}, it requires data be drawn from the stationary distribution.
%This issue is related to the problem with the IPS method that we previously mentioned in Section \ref{sec:intro}. For the IPS, off-policy data should reach the stationary distribution of the behavior policy and hence, in short horizon IPS is not going to perform well. 
In contrast, as shown in Figure \ref{fig:modelwin_b}, our black-box approach performance is independent of the horizon length, and substantially better.


\subsection{Classic Control}
We now focus on four classic control problems. We begin by briefly describing each problem and then compare the performance of our method with other approaches on these problems.  Note that for these problems are episodic, we convert them into infinite-horizon problems by resetting the state to a random start state once the episode terminates.

\paragraph{Pendulum.} In this environment, the goal is to control a pendulum in a vertical position. State variables are the pole angle $\theta$ and velocity $\dot{\theta}$. The action $a$ is the torque in the set $\{-2,-1,0,1,2\}$ applied to the base. We set the reward function to $-(\theta^2 + 0.1 \dot{\theta}^2 + 0.001 a^2)$.

\paragraph{Mountain Car.} For this problem, the goal is to drive up the car to top of a hill. Mountain Car has a state space of $\mathbb{R}^2$ (the position and speed of the car) and three possible actions (negative, positive, or zero acceleration). We set the reward to +100 when the car reaches the goal and -1 otherwise.

\paragraph{Cartpole.} The goal here is to prevent an attached pole to a cart from falling by changing the cart's velocity. Cartpole has a state space of $\mathbb{R}^4$ (cart position, velocity, pole angle and velocity) and two possible actions (moving left or right). Reward is -100 when the pole falls and +1 otherwise.

\paragraph{Acrobot.} In this problem, our goal is to swing a 2-link pendulum above the base. Acrobot has a state space of $\mathbb{R}^6$ ($\sin(.)$ and $\cos(.)$ of both angles and angular velocities) and three possible actions (applying +1, 0 or -1 torque on the joint). Reward is +100 for reaching the goal and -1 otherwise.


\begin{figure}
     \centering
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figs/cartpole_mean.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figs/pendulum_mean.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figs/mountaincar_mean.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figs/acrobot_mean.png}
     \end{subfigure}
        \caption{The RMSE of different methods w.r.t the target policy reward as we change the number of trajectories. Our black-box approach outperforms other methods on three problems.}
        \label{fig:RMSE}
\end{figure}

\iffalse
\begin{figure}[t!]
\centering
\subfigure{\includegraphics[width=0.24\textwidth]{Figs/cartpole_mean.png}}
\subfigure{\includegraphics[width=0.24\textwidth]{Figs/pendulum_mean.png}}
\subfigure{\includegraphics[width=0.24\textwidth]{Figs/mountaincar_mean.png}}
\subfigure{\includegraphics[width=0.24\textwidth]{Figs/acrobot_mean.png}}
\caption{The RMSE of different methods w.r.t the target policy reward as we change the number of trajectories. Our black-box approach outperforms other methods on three problems.}
\label{fig:RMSE}
\end{figure}
\fi


\begin{figure}
     \centering
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figs/cartpole_median.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figs/pendulum_median.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figs/mountaincar_median.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figs/acrobot_median.png}
     \end{subfigure}
        \caption{The median and error bars at \nth{25} and \nth{75} percentiles of different methods w.r.t the target policy reward as we change the number of trajectories. The trend of results is similar to Figure \ref{fig:RMSE}.}
        \label{fig:quantiles}
\end{figure}


\iffalse
\begin{figure}[t!]
\centering
\subfigure{\includegraphics[width=0.24\textwidth]{Figs/cartpole_median.png}}
\subfigure{\includegraphics[width=0.24\textwidth]{Figs/pendulum_median.png}}
\subfigure{\includegraphics[width=0.24\textwidth]{Figs/mountaincar_median.png}}
\subfigure{\includegraphics[width=0.24\textwidth]{Figs/acrobot_median.png}}
\caption{The median and error bars at \nth{25} and \nth{75} percentiles of different methods w.r.t the target policy reward as we change the number of trajectories. The trend of results is similar to Figure \ref{fig:RMSE}.}
\label{fig:quantiles}
\end{figure}
\fi

For each environment, we train a near-optimal policy $\pi_{+}$ using the {\em Neural Fitted Q Iteration} algorithm \cite{riedmiller2005neural}. We then set the behavior and target policies as $\pi_{\rm BEH}=\alpha_1 \pi_{+} + (1-\alpha_1) \pi_{-}$ and $\pi=\alpha_2 \pi_{+} + (1-\alpha_2) \pi_{-}$, where $\pi_{-}$ denotes a random policy, and $0\leq\alpha_1,\alpha_2\leq1$ are two constant values making the behavior policy distinct from the target policy. In our experiments, we set $\alpha_1=0.7$ and $\alpha_2=0.9$. In order to calculate the on-policy reward, we use a single trajectory collected by $\pi$ with $T_{\rm TAR}=50,000$. For off-policy data, we use multiple trajectories collected by $\pi_{\rm BEH}$ with $T_{\rm BEH}=200$. In all the cases, we use a 3-layer (having 30, 20, and 10 hidden neurons) feed-forward neural network with the sigmoid activation function as our parametric model in \eqref{eqn:bb-param}. For each setting, we report results based on 20 Monte-Carlo samples. 

Figure \ref{fig:RMSE} shows the $\log$ of RMSE w.r.t. the target policy reward as we change the number of trajectories collected by the behavior policy. We should note that all methods except the naive averaging method have hyperparameters to be tuned. For each method, the optimal set of parameters might depend on the number of trajectories (i.e., size of the training data). However, in order to avoid excessive tuning and to show how much each method is robust to a change in the number of trajectories, we only tune different methods based on 50 trajectories and use the same set of parameters for other settings. As we can see, the naive averaging performance is almost independent of the number of trajectories. Our method outperforms other approaches on three environments and it is only the Acrobot in which IPS performs comparably to our black-box approach. In order to have a robust evaluation against outliers, we have plotted the median and error bars at \nth{25} and \nth{75} percentiles in Figure \ref{fig:quantiles}. If we compare the Figures \ref{fig:RMSE} and \ref{fig:quantiles}, we notice that the trend of results is almost the same in both. In Appendix \ref{sec:sensitivity}, we have studied how changing $\alpha_1$ of the behavior policy affects the final RMSE.



\section{Conclusions}
In this paper, we presented a novel approach for solving the off-policy estimation problem in the long-horizon setting. Our method formulates the problem as solving for the fixed point of a ``backward flow'' operator. We showed that unlike previous works, our approach
does not require the knowledge of the behavior policy or stationary off-policy data. We presented
experimental results to show the effectiveness of our approach compared to previous baselines. In the future, we plan to use structural domain knowledge to improve the estimator and consider a random time horizon in episodic RL.


==> final/def.tex <==
%\newcommand{\E}{\mathbb{E}}
\newcommand{\defeq}{:=}
\newcommand{\bs}{\bar{s}}
\newcommand{\ba}{\bar{a}}
\newcommand{\Bop}{\mathcal{B}}
\newcommand{\Dset}{\mathcal{D}}
\newcommand{\Sset}{\mathcal{S}}
\newcommand{\Aset}{\mathcal{A}}
\newcommand{\SAset}{\Sset\times\Aset}
\newcommand{\Hset}{\mathcal{H}}
\newcommand{\Wset}{\mathcal{W}}
\newcommand{\Xset}{\mathcal{X}}
\newcommand{\Iset}{\mathcal{I}}
\newcommand{\Thetaset}{\Theta}
\newcommand{\Rset}{\mathbb{R}}
\newcommand{\D}{\mathbb{D}}
\newcommand{\Dist}[2]{\D(#1~\|~#2)}
\newcommand{\DistMMD}[2]{\D_{\kk}(#1~\|~#2)}
%\newcommand{\Dist}[2]{D(#1~\|~#2)}
%\newcommand{\DistMMD}[2]{D_\text{MMD}(#1~\|~#2)}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\mt}{{\operatorname{T}}}
%\newcommand{\argmin}{\operatorname{argmin}}
\newcommand{\Simplex}{\Delta}

\newcommand{\one}[1]{\mathbf{1}\{#1\}}

%%%%%%%%% QIANG +++++++
\newcommand{\Bpi}{\mathcal{B}_\pi}
\newcommand{\Bpihat}{\hat{\mathcal{B}}_\pi}
%\renewcommand{\Bop}{\Bpi}
%\renewcommand{\Bophat}{\hat{\Bpi}
\newcommand{\pibeh}{\pi_{\mathrm{BEH}}}
\renewcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\appref}[1]{Appendix~\ref{#1}}

\newcommand{\kf}{k}
\newcommand{\kfd}{k}
\newcommand{\kk}{\mathbf{k}} 
\newcommand{\kkf}[2]{\kk\left[#1;~#2\right]}
\newcommand{\sbar}{\bar{s}}
\newcommand{\abar}{\bar{a}}
\newcommand{\xbar}{\bar{x}}



\usepackage{color, xcolor}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{amsmath, amsthm, amsfonts, amssymb, mathtools}
\usepackage{cleveref}


\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}{Corollary}[section]
\newtheorem{lem}{Lemma}[section]
\newtheorem{ass}{Assumption}[section]
\newtheorem{mydef}{Definition}[section]
% \newtheorem{problem}[thm]{Problem} 
\newtheorem{exa}{Example} [section]
\newtheorem{pro}{Proposition}[section] 

%%%%%%%%%%%%%Define Remark environment %%%%%%%%%%%
\newtheorem{remark}{Remark}[section] 

%%%%%%%%%%%% Define homework environment %%%%%%%%%%
\usepackage{thmtools} 
\declaretheoremstyle[
  headfont=\color{magenta}\normalfont\bfseries,
  bodyfont=\color{black}\normalfont\itshape,
]{colored}

\declaretheorem[
  style=colored,
  name=Problem,  
  numberwithin=section, 
]{home}
%\newtheorem{home}{\textcolor{blue}{Homework}}[section]   
%\newtheorem{homeopt}[home]{Lemma} 

\declaretheorem[
  style=colored,
  name=Problem*, %(\textit{optional}),  
  numberwithin=section, 
]{homeopt}

% fix the spacing problem of theorem
\begingroup
    \makeatletter
    \@for\theoremstyle:=definition,remark,plain\do{%
        \expandafter\g@addto@macro\csname th@\theoremstyle\endcsname{%
            \addtolength\thm@preskip\parskip
            }%
        }
\endgroup


\usepackage{todonotes}
\newcommand{\ali}[1]{\todo{\textbf{AM}: #1}}
\newcommand{\lihong}[1]{\todo{\textbf{LL}: #1}}
\newcommand{\qiang}[1]{\todo{\textbf{QL}: #1}}
\newcommand{\denny}[1]{\todo{\textbf{DZ}: #1}}
\newcommand{\rev}[1]{\textcolor{blue}{#1}}

\renewcommand{\ali}[1]{}
\renewcommand{\lihong}[1]{}
\renewcommand{\qiang}[1]{}
\renewcommand{\denny}[1]{}


==> final/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

